Integrating Captive Portal Technology into Computer Science Education: A Modular, Hands-On Approach to Infrastructure

In this paper, we present an educational project aimed to introduce students to the technology behind Captive Portals infrastructures. For doing this, we developed a series of modules to emphasize each of the different aspects and features of this technology. The project is based on an open source implementation which is widely used in many computer network courses, making it well-suited and very appealing for instructors and practitioners in this field.

==> Makefile <==
NAME=CaptPort_main
TARGET=$(NAME).pdf
SOURCE=$(NAME).tex

DATE=`date +"%Y.%m%d"`
TARBALL=$(NAME)-$(DATE).tar.gz

JUNK=.aux .bbl .blg .dvi .log .nav .out .ps .pdf .snm .tex.backup .tex.bak .toc Notes.bib .spl

.PHONY: clean


$(TARGET): $(SOURCE) *tex 
	@pdflatex $(SOURCE)
	@bibtex $(NAME)
	@pdflatex $(SOURCE)
	@pdflatex $(SOURCE)


distrib:
	tar -cHvzf $(TARBALL)  *tex refs_CP.bib Makefile figs/ 

all: $(TARGET) $(TARGETa)

abs: $(TARGETa)

full: $(TARGET)

clean:
	@for ext in $(JUNK); do \
		rm -v $(NAME)$$ext; \
		rm -v $(NAMEa)$$ext; \
	done


==> modules.tex <==

%\section{Modules}
%\label{modules}


\include{table_modules}


%%%%

\subsection{Module 1 - TCP Sever and Client}\label{module-1---tcp-sever-and-client}

\subsubsection{Overview}\label{overview}

This module lays the foundational understanding of TCP connections,
vital for implementing captive portal projects. It aims to solidify
students' network programming skills and introduce them to Python coding
for network applications.

\subsubsection{Objectives}\label{objectives}

\begin{itemize}
%\tightlist
\item
  Comprehend the architecture and function of TCP servers and clients.
\item
  Understand the reason for using TCP to exchange information in Captive
  Portal.
\item
  Have a general understanding of the entire Captive Portal framework.
\end{itemize}

\subsubsection{Pre-requisites}\label{pre-requisites}

Basic understanding of TCP packets and python script.

\subsubsection{Implementations}\label{implementations}

Set up a TCP client in Mininet and enable it to communicate with a TCP
server hosted in the virtual machine.

\subsubsection{Learning Outcomes}\label{learning-outcomes}

Students will gain hands-on experience with network programming,
enhancing their understanding of how data is reliably transmitted across
a network.

%%%%

\subsection{Module 2 - SDN Switch}\label{module-2---sdn-switch}

\subsubsection{Overview}\label{overview-1}

Focuses on understanding Software-Defined Networking (SDN) controllers
and the manipulation of network traffic. Through hands-on practice with
the POX SDN Controller, students will learn how to program switches and
process network packets.

\subsubsection{Objectives}\label{objectives-1}

\begin{itemize}
%\tightlist
\item
  Achieve proficiency in utilizing the POX controller to program a
  network switch.
\item
  Explore the feasibility of modifying a standard switch to act as a
  captive portal.
\end{itemize}

\subsubsection{Pre-requisites}\label{pre-requisites-1}

Basic knowledge of networking concepts, including switches, MAC
addresses, and packet flow.

\subsubsection{Implementations}\label{implementations-1}

Students are provided with a basic POX code framework and tasked with
implementing a learning switch using POX, thus applying their
theoretical knowledge in a practical setting.

\subsubsection{Learning Outcomes}\label{learning-outcomes-1}

Enhanced understanding of SDN controllers and the ability to manipulate
network traffic for specific applications such as captive portals.


%%%%%

\subsection{Module 3 - DNS Server}\label{module-3---dns-server}

\subsubsection{Overview}\label{overview-2}

Introduces the functionality and implementation of DNS servers within
the context of captive portal technology. This module covers different
approaches to handling DNS requests, emphasizing hands-on experience
with DNS manipulation.

\subsection{Objectives}\label{objectives-2}

\begin{itemize}
%\tightlist
\item
  Learn to uniformly respond to all DNS queries with a specific IP
  address.
\item
  Develop skills to parse DNS requests, make requests on behalf of the
  user, and return genuine responses.
\item
  Modify DNS request destination IPs using iptables for direct server
  responses.
\end{itemize}

\subsubsection{Pre-requisites}\label{pre-requisites-2}

Basic knowledge of UDP packets and DNS protocols.

\subsubsection{Implementations}\label{implementations-2}

Students can explore one of three different DNS configuration methods,
from simple IP redirection to complex request handling and response
modification.

\subsubsection{Learning Outcomes}\label{learning-outcomes-2}

Students will understand how DNS servers can be manipulated to redirect
or handle requests in a captive portal setup.


%%%%%

\subsection{Module 4 - Web Server}\label{module-4---web-server}

\subsubsection{Overview}\label{overview-3}

Explores the deployment and configuration of a local web server to
interact directly with network requests, crucial for the operation of a
captive portal.

\subsubsection{Objectives}\label{objectives-3}

\begin{itemize}
%\tightlist
\item
  Set up and configure a local web server.
\item
  Use iptables to redirect web requests to the local server.
\end{itemize}

\subsubsection{Pre-requisites}\label{pre-requisites-3}

Basic understanding of web server operation and network request
handling.

\subsubsection{Implementations}\label{implementations-3}

Students will configure iptables to redirect web requests to a local
server, ensuring direct response capability.

\subsubsection{Learning Outcomes}\label{learning-outcomes-3}

Practical skills in web server setup and configuration, with an emphasis
on interaction with network requests in a captive portal context.

%%%%%

\subsection{Module 5 - Mininet Script}\label{module-5---mininet-script}


\subsubsection{Overview}\label{overview-4}

Delves into network simulation using Mininet, teaching students to
construct and modify network topologies to route user requests through
specific servers, mimicking a captive portal environment.


\subsubsection{Objectives}\label{objectives-4}

\begin{itemize}
%\tightlist
\item
  Understand network structure and the necessary modifications for
  captive portal functionality.
\item
  Learn to use Mininet for creating and testing network topologies.
\end{itemize}


\subsubsection{Pre-requisites}\label{pre-requisites-4}

Basic knowledge of network topology and mininet.


\subsubsection{Implementations}\label{implementations-4}

Students have the flexibility to design the network according to the
requirements of the captive portal setup they envision.


\subsubsection{Learning Outcomes}\label{learning-outcomes-4}

Ability to simulate and test network configurations, crucial for the
development and deployment of captive portal technologies.

%%%%%%


==> tools.tex <==
%---------------- show page layout. don't use in a real document!
\usepackage{showframe}
\renewcommand\ShowFrameLinethickness{0.15pt}
\renewcommand*\ShowFrameColor{\color{red}}
%---------------------------------------------------------------%

